CountCLIP -- [Re] Teaching CLIP to Count to Ten

Large vision-language models (VLMs) are shown to learn rich joint image-text representations enabling high performances in relevant downstream tasks. However, they fail to showcase their quantitative understanding of objects, and they lack good counting-aware representation. This paper conducts a reproducibility study of 'Teaching CLIP to Count to Ten' (Paiss et al., 2023), which presents a method to finetune a CLIP model (Radford et al., 2021) to improve zero-shot counting accuracy in an image while maintaining the performance for zero-shot classification by introducing a counting-contrastive loss term. We improve the model's performance on a smaller subset of their training data with lower computational resources. We verify these claims by reproducing their study with our own code. The implementation can be found at https://github.com/SforAiDl/CountCLIP.

==> metadata.tex <==
% DO NOT EDIT - automatically generated from metadata.yaml

\def \codeURL{https://github.com/SforAiDl/CountCLIP}
\def \codeDOI{}
\def \codeSWH{}
\def \dataURL{https://doi.org/10.5281/zenodo.10981852}
\def \dataDOI{10.5281/zenodo.10981852}
\def \editorNAME{}
\def \editorORCID{}
\def \reviewerINAME{}
\def \reviewerIORCID{}
\def \reviewerIINAME{}
\def \reviewerIIORCID{}
\def \dateRECEIVED{01 November 2018}
\def \dateACCEPTED{}
\def \datePUBLISHED{}
\def \articleTITLE{[Re] Teaching CLIP to Count to Ten}
\def \articleTYPE{Replication}
\def \articleDOMAIN{Computer Vision}
\def \articleBIBLIOGRAPHY{bibliography.bib}
\def \articleYEAR{2024}
\def \reviewURL{}
\def \articleABSTRACT{Large vision-language models (VLMs), such as CLIP, learn rich joint image-text representations, facilitating advances in numerous downstream tasks, including zero-shot classification and text-to-image generation. Nevertheless, existing VLMs exhibit a prominent well-documented limitation - they fail to encapsulate compositional concepts such as counting. We introduce a simple yet effective method to improve the quantitative understanding of VLMs, while maintaining their overall performance on common benchmarks. Specifically, we propose a new counting-contrastive loss used to finetune a pre-trained VLM in tandem with its original objective. Our counting loss is deployed over automatically-created counterfactual examples, each consisting of an image and a caption containing an incorrect object count. For example, an image depicting three dogs is paired with the caption "Six dogs playing in the yard". Our loss encourages discrimination between the correct caption and its counterfactual variant which serves as a hard negative example. To the best of our knowledge, this work is the first to extend CLIP's capabilities to object counting. Furthermore, we introduce "CountBench" - a new image-text counting benchmark for evaluating a model's understanding of object counting. We demonstrate a significant improvement over state-of-the-art baseline models on this task. Finally, we leverage our count-aware CLIP model for image retrieval and text-conditioned image generation, demonstrating that our model can produce specific counts of objects more reliably than existing ones.}
\def \replicationCITE{Teaching CLIP to Count to Ten}
\def \replicationBIB{paiss2023teaching}
\def \replicationURL{https://arxiv.org/pdf/2302.12066}
\def \replicationDOI{https://doi.org/10.48550/arXiv.2302.12066}
\def \contactNAME{Harshvardhan Mestha}
\def \contactEMAIL{harshvardhanmestha@yahoo.com}
\def \articleKEYWORDS{rescience c, rescience x, pytorch, VLMs, CLIP, Computer Vision}
\def \journalNAME{ReScience C}
\def \journalVOLUME{4}
\def \journalISSUE{1}
\def \articleNUMBER{}
\def \articleDOI{}
\def \authorsFULL{Harshvardhan Mestha et al.}
\def \authorsABBRV{H. Mestha et al.}
\def \authorsSHORT{Mestha et al.}
\title{\articleTITLE}
\date{}
\author[1,2]{Harshvardhan Mestha}
\author[1,2]{Tejas Agrawal}
\author[1,2]{Karan Bania}
\author[1,2]{Shreyas V}
\author[1,2]{Yash Bhisikar}
\affil[1]{SAiDL, Goa, India}
\affil[2]{BITS Pilani, Goa, India}

